Topological Quantum Computation with Gapped Boundaries

This paper studies fault-tolerant quantum computation with gapped boundaries. We first introduce gapped boundaries of Kitaev's quantum double models for Dijkgraaf-Witten theories using their Hamiltonian realizations. We classify the elementary excitations on the boundary, and systematically describe the bulk-to-boundary condensation procedure. We also provide a commuting Hamiltonian to realize defects between boundaries in any quantum double model. Next, we present the algebraic/categorical structure of gapped boundaries and boundary defects, which will be used to describe topologically protected operations and obtain quantum gates. To demonstrate a potential physical realization, we provide quantum circuits for surface codes that can perform all basic operations on gapped boundaries. Finally, we show how gapped boundaries of the abelian theory $\mathfrak{D}(\mathbb{Z}_3)$ can be used to perform universal quantum computation.

==> ch5/ch5_4/ch5_4_v1.tex <==
\subsection{Topological Charge Measurement}
\label{sec:measurement}

Given a topological order $\B=\ZZ{(\CC)}$ on a rectangle $Y$ with $n$ holes $\mfh_i,i=1,...,n$ labeled by Lagrangian algebras $\A_i$ and trivial charge at the outermost boundary.  Then the ground state manifold is $\textrm{Hom}(1, \otimes_i \A_i)$.  For the Dijkgraaf-Witten theory, all unitary gates from tunneling operators and braidings form a finite group, therefore cannot form universal gate sets.  In this section, we consider a physically reasonable protocol to obtain more gates---topological charge measurement as inspired by [].

Any closed loop labeled by anyons of $\B$ or arc connecting different holes labeled by anyons from the corresponding boundary condensates generates a generalized Wilson operator on $\textrm{Hom}(1, \otimes_i \A_i)$.  All such operators generate an algebra $\mathcal{M}(\B,\A_i)$, which will be called the Wilson operator algebra.  The ground state manifold $\textrm{Hom}(1, \otimes_i \A_i)$ is a representation of the Wilson operator algebra, therefore the Wilson operator algebra is an emergent symmetry algebra of the theory at low energy.

We posit that any Hermitian operator $\mathcal{O}\in \mathcal{M}(\B,\A_i)$ can be measured, and $\mathcal{O}$ will be called a topological charge measurement operator.  The corresponding projective measurement $P_\mathcal{O}$ will be called a topological charge measurement, and  

Let $D(Y)$ be the closed surface obtained by gluing two copies of $Y$ along the corresponding boundaries.  Any generic closed simple loop $l$ on $D(Y)$ can be projected onto $Y$, which results in a knot diagram on $Y$.  In the case $\CC$ is modular, then as explained in [], we can measure the flux through the loop $l$ for the topological order $\CC$ on $D(Y)$.  This theory can be generalized partially to the case $\CC$ is not modular but abelian [].  Our postulate is a generalization of these results.

For systematical topological charge measurement, we choose a maximal collection of loops circling the holes and arcs connecting adjacent holes and use tunneling operators obtained from labeling all the loops and arcs as a bases to generate $\mathcal{M}(\B,\A_i)$.  Then each knot diagram in $Y$ can be resolved using the graphical calculus to a linear combinations of these loop and arc operators.   In general, any operator $h$ can be used to form a topological charge measurement operator $h+{h}^{\dagger}$, though maybe unphysical.

To be more physical, we will consider only operators which are monomials of basis operators.   Let $H_i, O_i$ be the complete collection of basis operators such that $H_i$ are Hermitian and $O_i$ are non-Hermitian.  All $H_i$ give rise to topological charge measurements. 

\subsubsection{Topological charge projection}

Suppose $\B=\ZZ(\CC)$ represents a topological order such that $\CC$ is also modular.  Then there is a TQFT from the modular category $\CC$.  Physically, a Wilson operator along a simple closed loop $l$ on $D(Y)$ measures charges through the loop $l$.  If $l$ is projected on a closed loop around a hole, then the Wilson operator measuring charge $a$ through $l$ in $D(Y)$ leads to a topological charge measurement $P^a_l=\sum_{x\in L_\CC}s_{0a}s_{xa}^{*}W_x(l)$, where $L_\CC$ is the label set of $\CC$ and $s_{ab}$ is the modular $s$-matrix of $\CC$.  If $l$ is projected to an arc $\gamma$, then the topological charge projection operator is $P^a_l=\sum_{x\in L_\CC}s_{0a}s_{xa}^{*}W_{xx^*}(l)$.

In [], it is shown that topological charge projections can be used to generate all the mapping class group representations $V_{\CC}(Y)$ of a closed surface $Y$ from the modular category $\CC$.

\subsubsection{Physicallyl implementable topological charge measurement} Given a product of some basis Hermitian operators $H_{i_j}$ of the Wilson operator algebra such that $H_{i_1}\cdots H_{i_k}=\alpha H_{i_k}\cdots H_{i_1}$ for some phase $\alpha$, then the Hermitian operator $\sqrt{\alpha}H_{i_1}\cdots H_{i_k}$ is a topological charge measurement operator.  


==> ch6/ch6_4/ch6_4.tex <==
\subsection{Anyonic Quantum Computing using gapped boundaries}
\label{sec:gapped-boundaries-ancillas}

\subsubsection{Braiding boundary defects and anyons with defects}

Given a topological order $\B=\ZZ(\mathcal{C})$.  Let $\{\mathcal{M}_i\}$ be all of $\mathcal{C}$'s distinct indecomposable module categories and $\mathcal{C}_{ij}=\textrm{Fun}_{\mathcal{C}}(\mathcal{M}_i,\mathcal{M}_j)$.  Then $\{\mathcal{C}_{ij}\}$ form a multi-fusion category $\mathfrak{C}$.  
Its Drinfeld center $\ZZ(\mathfrak{C})=\ZZ(\mathcal{C}_{ii})=\ZZ(\mathcal{C})$ for any $i$.  Fixed two boundary types $\M_i$ and $\M_j$.  The boundary defects between $\M_i$ and $\M_j$ is the functor category $\mathcal{C}_{ij}$.  For the Dijkgraaf-Witten theory, one of the triangles in ??? is a functor $F:\M_{ij}\rightarrow \M_{ij}\boxtimes \M_{ij}^{\textrm{op}}\rightarrow \ZZ(\M)$, and in general $F$ sends $\mathcal{M}_{ij}$ to $\mathcal{M}_{ij}\otimes 1$ .  Therefore, the defects in $\M_{ij}$, identified as their images by $F$ in $\ZZ(\M)$, can be braided and can also be braided with bulk anyons of $\B$.



==> ch7/ch7_main/ch7_v1.tex <==
\section{Conclusions}
\label{sec:conclusions}

Based on Kitaev's quantum double models and Bombin and Martin-Delgado's two parameter generalization, we find exactly solvable Hamiltonian realizations of both gapped boundaries and defects between them in Dijkgraaf-Witten theories. By combining with an algebraic model, we develop a microscopic theory for gapped boundaries and defects between boundaries that allows us to compute topological operations such as braiding on these new topological degeneracy.  We design qubit and qutrit topological quantum computing models using $\mathfrak{D}(S_3)$. We then develop a universal qutrit topological quantum computing model using $\mathfrak{D}(Z_3)$.

We would like to conclude by considering several potential areas to generalize our work. First, many physics papers have studied gapped domain walls between different topological phases. While gapped boundaries are often considered as a special case of gapped domain walls, by the folding trick \cite{KitaevKong}, they also completely cover the domain wall theory mathematically. Physically, however, it is still interesting to analyze the general gapped domain walls following our work.

Another direction is to generalize our theory to the Levin-Wen model, using quantum groupoids.

The most interesting question that we have not touched on is the stability of topological degeneracy.  Once our Hamiltonian moves off the fixed-point, finite-size splitting of the degeneracy would occur.  It would be interesting to study the energy spitting of ground state degeneracy numerically under small perturbations.

Gapped boundaries and symmetry defects significantly enrich the physics of topological phases of matter in two spacial dimensions.  Their higher dimensional generalizations would be also very interesting.  As in the case of non-abelian anyons, experimental confirmation of non-abelian defects such as parafermion zero modes would be a landmark in condensed matter physics.
